Striking Gold in Advertising: Standardization and Exploration of Ad Text Generation

In response to the limitations of manual ad creation, significant research has been conducted in the field of automatic ad text generation (ATG). However, the lack of comprehensive benchmarks and well-defined problem sets has made comparing different methods challenging. To tackle these challenges, we standardize the task of ATG and propose a first benchmark dataset, CAMERA, carefully designed and enabling the utilization of multi-modal information and facilitating industry-wise evaluations. Our extensive experiments with a variety of nine baselines, from classical methods to state-of-the-art models including large language models (LLMs), show the current state and the remaining challenges. We also explore how existing metrics in ATG and an LLM-based evaluator align with human evaluations.

==> figures/fig_gpt4-preference.tex <==
\begin{figure}[t]
 \centering
  \includegraphics[width=0.85\linewidth]{figures/gpt4_preference.png}
 \caption{Preference evaluation using GPT-4 as the annotator.}
 \label{fig:gpt4_preference}
\end{figure}

==> figures/fig_industry-wise_eval.tex <==

\begin{figure}[t]
    \begin{tabular}{c}
    
    %------------------- Precision ---------------------
  \begin{minipage}[]{0.45\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/B-4.pdf}    
    \subcaption{B-4}\label{fig:blue}
  \end{minipage}  


    % % ------ 中央スペース---------
    % \begin{minipage}{0.02\hsize}
    %     \hspace{1mm}
    % \end{minipage}
    
   %------------------- Recall ---------------------
    \begin{minipage}[]{0.45\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/R-1.pdf}    
    \subcaption{R-1}\label{fig:rouge}
  \end{minipage}



  \end{tabular}
  \caption{Industry-wise evaluation.}
  \label{fig:industry_wise_eval}
\end{figure}


% \begin{figure*}[t]
%  \begin{minipage}{0.33\hsize}
%   \begin{center}
%    \includegraphics[width=40mm]{figures/B-4.pdf}
%   \end{center}
%   \caption{B-4}
%   \label{fig:one}
%  \end{minipage}
%  \begin{minipage}{0.33\hsize}
%  \begin{center}
%   \includegraphics[width=40mm]{figures/R-1.pdf}
%  \end{center}
%   \caption{R-1}
%   \label{fig:two}
%  \end{minipage}
%  \begin{minipage}{0.33\hsize}
%  \begin{center}
%   \includegraphics[width=40mm]{figures/BERT-Score.pdf}
%  \end{center}
%   \caption{BERT-Score}
%   \label{fig:three}
%  \end{minipage}
% \end{figure*}


% \begin{figure*}[t]
%     \begin{tabular}{c}
    
%     %------------------- B-4 ---------------------
%   \begin{minipage}[]{0.33\linewidth}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/B-4.pdf}    
%     \subcaption{B-4}\label{fig:blue}
%   \end{minipage}  


%    %------------------- R-1 ---------------------
%     \begin{minipage}[]{0.33\linewidth}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/R-1.pdf}    
%     \subcaption{R-1}\label{fig:rouge}
%   \end{minipage}


%    %------------------- B-F1 ---------------------
%     \begin{minipage}[]{0.33\linewidth}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/BERT-Score.pdf}    
%     \subcaption{BS}\label{fig:bertscore}
%   \end{minipage}



%   \end{tabular}
%   \caption{Industry-wise evaluation for each metrics.}
%   \label{fig:industry_wise_eval}
% \end{figure*}

==> figures/fig_model_length_bin.tex <==
\begin{figure*}[t]
 \centering
  \includegraphics[width=0.85\linewidth]{figures/models_bins_iso.png}
 \caption{Histogram of output length for each model}
 \label{fig:histgram}
\end{figure*}

==> figures/fig_window-analysis.tex <==
\begin{figure*}[t]
 \centering
  \includegraphics[width=0.9\linewidth]{figures/window_analysis.png}
 \caption{Window analysis}
 \label{fig:window_analysis}
\end{figure*}

==> tables/tab_CAMERA_example.tex <==


\begin{table*}[th]
\centering
\small
\begin{tabular}{lcl}
\toprule
\bf LP description    & \multicolumn{1}{l}{\bf User query} & \bf Ad text   \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} CardLoanDiagnosis.com   \\ Diagnosis of \bgfa{instant}loan cards!    \\ \bgfb{3 recommended} companies  \\ to borrow money \bgfa{now}! \end{tabular}} & \multirow{4}{*}{ORIX Card Loan}   & 1. [Official] \bgfb{Top 3 Popular} Card Loans  \\
                &             & 2. \bgfc{Easily} diagnose \bgfb{recommended} card loans \\
                 &                           & 3. Diagnose Cards Available for \bgfa{Same-Day} Borrowing!    \\
              &                           &  4. Get Financing in \bgfa{as Fast as 30 Minutes} \bgfc{Online}!  \\ 
\bottomrule           
\end{tabular}
\end{table*}



